Shallow and Deep Convolutional Networks for Saliency Prediction

The prediction of salient areas in images has been traditionally addressed with hand-crafted features based on neuroscience principles. This paper, however, addresses the problem with a completely data-driven approach by training a convolutional neural network (convnet). The learning process is formulated as a minimization of a loss function that measures the Euclidean distance of the predicted saliency map with the provided ground truth. The recent publication of large datasets of saliency prediction has provided enough data to train end-to-end architectures that are both fast and accurate. Two designs are proposed: a shallow convnet trained from scratch, and a another deeper solution whose first three layers are adapted from another network trained for classification. To the authors knowledge, these are the first end-to-end CNNs trained and tested for the purpose of saliency prediction.

==> 7_additional.tex <==
\section{Additional material}

Table \ref{tab:light} contains the details for the memory requirements of the light network. As in most ConvNets, the highest memory requirements correspond to the early convolutional layers, while the largest amount of parameters are associated to the fully connected layers at the deepest level of the network.

\begin{table*}
\begin{center}
\begin{tabular}{|l|c|c|}
\hline
Layer		& 	Blob Data Size			 & Filter Weights   \\
			& 	[Width x Height x Depth] & [( convX x convY x DepthIn ) x Depth]    \\
\hline
input 		& 96x96x3 = 27,648			& 0 \\
conv5-32 	& 92x92x32	= 270,848 		& (5x5x3)x32+32= 2,400\\
maxpool2 	& 46x46x32 	= 67,712		& 0 \\
conv3-64 	& 44x44x64  = 123,904		& (3x3x32)x64+64= 18,496\\
maxpool2 	& 22x22x64  = 30,976		& 0 \\
conv3-128 	& 20x20x128  = 30,976		& (3x3x64)x128+128= 73,856 \\
maxpool2 	& 10x10x128  = 12,800		& 0 \\
FC-4608 	& 1x1x4608  = 4,608			& (1x1x12,800)x4,608+4,608= 58,987,008\\
slice1 		& 1x1x2304  = 2,304			& 0 \\
slice2 		& 1x1x2304  = 2,304			& 0 \\
maxout 		& 1x1x2304  = 2,304			& 0 \\
FC-2304 	& 1x1x2304  = 2,304			& (1x1x2,304)x2,304+2,304= 5,310,720\\
output		& 1x48x48 = 2,304			&   \\
\hline
Total 		& 601,216					& 64,392,512 \\
Memory (train) 	& 4.58 MB				& - \\
Memory (test) 	& 2.29 MB 				& 246 MB \\
\hline
\end{tabular}
\end{center}
\caption{Memory requirements for the proposed shallow ConvNet.}
\label{tab:light}
\end{table*}
